Portfolio Decisions and Brain Reactions via the CEAD method

Decision making can be a complex process requiring the integration of several attributes of choice options. Understanding the neural processes underlying (uncertain) investment decisions is an important topic in neuroeconomics. We analyzed functional magnetic resonance imaging (fMRI) data from an investment decision study for stimulus-related effects. We propose a new technique for identifying activated brain regions: Cluster, Estimation, Activation and Decision (CEAD) method. Our analysis is focused on clusters of voxels rather than voxel units. Thus, we achieve a higher signal to noise ratio within the unit tested and a smaller number of hypothesis tests compared with the often used General Linear Model (GLM). We propose to first conduct the brain parcellation by applying spatially constrained spectral clustering. The information within each cluster can then be extracted by the flexible Dynamic Semiparametric Factor Model (DSFM) dimension reduction technique and finally be tested for differences in activation between conditions. This sequence of Cluster, Estimation, Activation and Decision admits a model-free analysis of the local fMRI signal. Applying a GLM on the DSFM-based time series resulted in a significant correlation between the risk of choice options and changes in fMRI signal in the anterior insula and dorsomedial prefrontal cortex. Additionally, individual differences in decision-related reactions within the DSFM time series predicted individual differences in risk attitudes as modeled with the framework of the mean-variance model.

==> defs.tex <==
% some definitions of colors
% require the xcolor-package

\xdefinecolor{isered}{rgb}{0.9,0,0}

\xdefinecolor{iseblue}{rgb}{0,0.35,0.62}
\xdefinecolor{linkblue}{rgb}{0,0.35,0.62}
\xdefinecolor{navyblue}{rgb}{0,0.35,0.62}

%\xdefinecolor{linkblue}{rgb}{1,0,1}
%\xdefinecolor{navyblue}{rgb}{0,0,0.8}


\xdefinecolor{isegreen}{rgb}{0,0.4,0}
\xdefinecolor{darkgreen}{rgb}{0,.75,0}

%20,99,50
\xdefinecolor{isegray}{rgb}{0.5,0.5,0.5}

% color definitions for listings:
\definecolor{hellgelb}{rgb}{1,1,0.7}
\definecolor{colKeys}{rgb}{0,0.35,0.62}
\definecolor{colIdentifier}{rgb}{0,0,0}
\definecolor{colComments}{rgb}{1,0,0}
\definecolor{colString}{rgb}{0,0.5,0}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Defined by Song, be CAREFUL when use it.
\newcommand{\xy}{\{(X_i, Y_i)\}_{i=1}^n}
\newcommand{\lnh}{l_{n,h}}
\newcommand{\lng}{l_{n,g}}


%===================================================================
%Variable Notations
%===================================================================

\newcommand{\nit}{\mathbb{N}}
\renewcommand{\i}{\mbox{\bf i}}
\newcommand{\CO}{{\mathcal{O}}}
\newcommand{\rit}{\mathbb{R}}
\newcommand{\zit}{\mathbb{Z}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\tr}{\mathop{\rm{tr}}}
\newcommand{\diag}{\mathop{\rm{diag}}}
\newcommand{\rank}{\mathop{\rm{rank}}}
\newcommand{\Var}{\mathop{\mbox{\sf Var}}}
\newcommand{\var}{\mathop{\mbox{\sf Var}}}
\newcommand{\cov}{\mathop{\mbox{Cov}}}
\newcommand{\E}{\mathop{\mbox{\sf E}}}     % ISE
\renewcommand{\P}{\operatorname{P}}            % ISE
\newcommand{\Corr}{\mathop{\mbox{Corr}}}
\def\N{\mbox{N}}            % Normal distribution
\def\std{\mathop{\mbox{Std}}}            %standard deviation
\newcommand{\IF}{\boldsymbol{1}}    % indicator function
\def\Co{{\scriptstyle \mathcal{O}}} % small {\cal o}
\def\defeq{\stackrel{\mathrm{def}}{=}}  % for definition


%%corollary
%\newtheorem{corollary}{\corollaryname}[section]
%\newtheorem{corollary}[theorem]{COROLLARY}
%proof
%SK \newenvironment{proof}{\noindent{\bf Proof:}\newline\noindent}
%SK {\quad ${\Box}$ \newline}
%\newenvironment{proof}{\noindent{\bf \proofname.}}%\newline\noindent}
%{\quad ${\Box}$ \newline}
%
%\def\proofname{PROOF}
%\def\corollaryname{COROLLARY}
%\def\corollaryname{PROPOSITION}
%\def\remarkname{REMARK}


%theorem
% \newtheorem{theorem}{THEOREM}[chapter]

%\newtheorem{theorem}{THEOREM}[section]
%\newtheorem{corollary}{COROLLARY}[section]
%\newtheorem{proposition}{PROPOSITION}[section]
%\newtheorem{lemma}{LEMMA}[section]
%
%\def\definitionname{DEFINITION}
%\newtheorem{testproblem}{TEST PROBLEM}

%\newtheorem{testproblem}{\testproblemname}
%\def\testproblemname{\bf\sffamily TEST PROBLEM}

%\def\testproblemname{TEST PROBLEM}

%remark
%\newtheorem{remark}{\remarkname}[section]
%\newtheorem{definition}{\definitionname}[section]



%===================================================================
%Variable Notations
%===================================================================
\def\boxit#1#2#3{\hbox{\vrule width #2               %The left line
                     \vtop{%
                             \vbox{\hrule  height #2 \kern#1 %The upper line and space
                           \hbox{\kern#1 #3\kern#1}  %Right space; text; left space
                          }%
                     \kern#1 \hrule  height #2   %The bottom line and space
                  }%
                         \vrule width #2             %The right line
                      } %
                  }


\newcommand{\display}[2][4in]{%
\par\vspace{2ex}\begin{center}\mbox{}
    \boxit{10pt}{0.5pt}{
    \textwidth=#1
    \begin{minipage}[c]\textwidth
        \begin{center}{#2}
        \end{center}
    \end{minipage}}
    \end{center}
    \par\vspace{2ex}}

     \def\eps{\ensuremath{\varepsilon}}
\def\iid{i.i.d.\xspace }
\def\argmax{\mathop{\mbox{arg\,max}}}
\def\argmin{\mathop{\mbox{arg\,min}}}
\def\ind{\IF}
\def\en{\infty}
\def\summ#1#2#3{\sum_{#1=#2}^{#3}}
\def\noframe{}
\newcommand{\eqsplit}[2][*]%
  {\ifthenelse{\equal{#1}{*} \or\equal{#1}{<???>}
                     \or\equal{#1}{nn} \or\equal{#1}{ } \or\equal{#1}{}}
    { \begin{align*}%
         #2 %
         \end{align*}%
        }
    {\begin{equation}\label{#1}\begin{split}\allowdisplaybreaks%
         #2%
         \end{split}\end{equation}
        }
  }

\def\del{\delta}
\def\al{\alpha}
\def\ti{\tilde}
\def\bb#1{\mathbb{#1}}
     \def\bbs{\ensuremath{{\bb S}}}
\def\t{^{\scriptstyle{\mathsf{T}}} \hspace{-0.15em}}
\renewcommand{\O}{\CO}
\def\sfa{\scalefont{0.6}}
\def\sfb{\scalefont{1.6666666666}}
\renewcommand{\o}{\Co}

\newcounter{margc}
\def\marg#1{\stepcounter{margc}\Blue$\dag_{\arabic{margc}}$\endBlue\marginpar{\Blue\arabic{margc} %
    \boxit{3pt}{1pt}{%
        \textwidth = 1.2\marginparwidth
        \begin{minipage}%
            \textwidth\begin{sloppypar}\raggedright%
            \tiny \hspace{
0pt}#1\end{sloppypar}%
        \end{minipage}%
    }%
    }}
\def\eqdef{\stackrel{\rm def}{=}}

%%\renewenvironment{Blue}{\special{color push Blue}}{\special{color pop}}
%\renewenvironment{Blue}{\color{blue}}{\color{black}}
%\renewenvironment{Emerald}{\special{color push Emerald}}{\special{color pop}}
%%\renewenvironment{Red}{\special{color push  Red}}{\special{color pop}}
%\renewenvironment{Red}{\color{red}}{\color{black}}
%\renewenvironment{Cyan}{\special{color push Cyan}}{\special{color pop}}
%\renewenvironment{textColor}[1]{\special{color push #1}}{\special{color pop}}
%\renewenvironment{Yellow}{\special{color push  Yellow}}{\special{color pop}}
%\renewenvironment{Black}{\special{color push  Black}}{\special{color pop}}
%\renewenvironment{Gray}{\special{color push  Gray}}{\special{color pop}}


==> fmri_paper_20141015 copy/defs.tex <==
% some definitions of colors
% require the xcolor-package

\xdefinecolor{isered}{rgb}{0.9,0,0}

\xdefinecolor{iseblue}{rgb}{0,0.35,0.62}
\xdefinecolor{linkblue}{rgb}{0,0.35,0.62}
\xdefinecolor{navyblue}{rgb}{0,0.35,0.62}

%\xdefinecolor{linkblue}{rgb}{1,0,1}
%\xdefinecolor{navyblue}{rgb}{0,0,0.8}


\xdefinecolor{isegreen}{rgb}{0,0.4,0}
\xdefinecolor{darkgreen}{rgb}{0,.75,0}

%20,99,50
\xdefinecolor{isegray}{rgb}{0.5,0.5,0.5}

% color definitions for listings:
\definecolor{hellgelb}{rgb}{1,1,0.7}
\definecolor{colKeys}{rgb}{0,0.35,0.62}
\definecolor{colIdentifier}{rgb}{0,0,0}
\definecolor{colComments}{rgb}{1,0,0}
\definecolor{colString}{rgb}{0,0.5,0}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Defined by Song, be CAREFUL when use it.
\newcommand{\xy}{\{(X_i, Y_i)\}_{i=1}^n}
\newcommand{\lnh}{l_{n,h}}
\newcommand{\lng}{l_{n,g}}


%===================================================================
%Variable Notations
%===================================================================

\newcommand{\nit}{\mathbb{N}}
\renewcommand{\i}{\mbox{\bf i}}
\newcommand{\CO}{{\mathcal{O}}}
\newcommand{\rit}{\mathbb{R}}
\newcommand{\zit}{\mathbb{Z}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\tr}{\mathop{\rm{tr}}}
\newcommand{\diag}{\mathop{\rm{diag}}}
\newcommand{\rank}{\mathop{\rm{rank}}}
\newcommand{\Var}{\mathop{\mbox{\sf Var}}}
\newcommand{\var}{\mathop{\mbox{\sf Var}}}
\newcommand{\cov}{\mathop{\mbox{Cov}}}
\newcommand{\E}{\mathop{\mbox{\sf E}}}     % ISE
\renewcommand{\P}{\operatorname{P}}            % ISE
\newcommand{\Corr}{\mathop{\mbox{Corr}}}
\def\N{\mbox{N}}            % Normal distribution
\def\std{\mathop{\mbox{Std}}}            %standard deviation
\newcommand{\IF}{\boldsymbol{1}}    % indicator function
\def\Co{{\scriptstyle \mathcal{O}}} % small {\cal o}
\def\defeq{\stackrel{\mathrm{def}}{=}}  % for definition


%%corollary
%\newtheorem{corollary}{\corollaryname}[section]
%\newtheorem{corollary}[theorem]{COROLLARY}
%proof
%SK \newenvironment{proof}{\noindent{\bf Proof:}\newline\noindent}
%SK {\quad ${\Box}$ \newline}
%\newenvironment{proof}{\noindent{\bf \proofname.}}%\newline\noindent}
%{\quad ${\Box}$ \newline}
%
%\def\proofname{PROOF}
%\def\corollaryname{COROLLARY}
%\def\corollaryname{PROPOSITION}
%\def\remarkname{REMARK}


%theorem
% \newtheorem{theorem}{THEOREM}[chapter]

%\newtheorem{theorem}{THEOREM}[section]
%\newtheorem{corollary}{COROLLARY}[section]
%\newtheorem{proposition}{PROPOSITION}[section]
%\newtheorem{lemma}{LEMMA}[section]
%
%\def\definitionname{DEFINITION}
%\newtheorem{testproblem}{TEST PROBLEM}

%\newtheorem{testproblem}{\testproblemname}
%\def\testproblemname{\bf\sffamily TEST PROBLEM}

%\def\testproblemname{TEST PROBLEM}

%remark
%\newtheorem{remark}{\remarkname}[section]
%\newtheorem{definition}{\definitionname}[section]



%===================================================================
%Variable Notations
%===================================================================
\def\boxit#1#2#3{\hbox{\vrule width #2               %The left line
                     \vtop{%
                             \vbox{\hrule  height #2 \kern#1 %The upper line and space
                           \hbox{\kern#1 #3\kern#1}  %Right space; text; left space
                          }%
                     \kern#1 \hrule  height #2   %The bottom line and space
                  }%
                         \vrule width #2             %The right line
                      } %
                  }


\newcommand{\display}[2][4in]{%
\par\vspace{2ex}\begin{center}\mbox{}
    \boxit{10pt}{0.5pt}{
    \textwidth=#1
    \begin{minipage}[c]\textwidth
        \begin{center}{#2}
        \end{center}
    \end{minipage}}
    \end{center}
    \par\vspace{2ex}}

     \def\eps{\ensuremath{\varepsilon}}
\def\iid{i.i.d.\xspace }
\def\argmax{\mathop{\mbox{arg\,max}}}
\def\argmin{\mathop{\mbox{arg\,min}}}
\def\ind{\IF}
\def\en{\infty}
\def\summ#1#2#3{\sum_{#1=#2}^{#3}}
\def\noframe{}
\newcommand{\eqsplit}[2][*]%
  {\ifthenelse{\equal{#1}{*} \or\equal{#1}{<???>}
                     \or\equal{#1}{nn} \or\equal{#1}{ } \or\equal{#1}{}}
    { \begin{align*}%
         #2 %
         \end{align*}%
        }
    {\begin{equation}\label{#1}\begin{split}\allowdisplaybreaks%
         #2%
         \end{split}\end{equation}
        }
  }

\def\del{\delta}
\def\al{\alpha}
\def\ti{\tilde}
\def\bb#1{\mathbb{#1}}
     \def\bbs{\ensuremath{{\bb S}}}
\def\t{^{\scriptstyle{\mathsf{T}}} \hspace{-0.15em}}
\renewcommand{\O}{\CO}
\def\sfa{\scalefont{0.6}}
\def\sfb{\scalefont{1.6666666666}}
\renewcommand{\o}{\Co}

\newcounter{margc}
\def\marg#1{\stepcounter{margc}\Blue$\dag_{\arabic{margc}}$\endBlue\marginpar{\Blue\arabic{margc} %
    \boxit{3pt}{1pt}{%
        \textwidth = 1.2\marginparwidth
        \begin{minipage}%
            \textwidth\begin{sloppypar}\raggedright%
            \tiny \hspace{
0pt}#1\end{sloppypar}%
        \end{minipage}%
    }%
    }}
\def\eqdef{\stackrel{\rm def}{=}}

%%\renewenvironment{Blue}{\special{color push Blue}}{\special{color pop}}
%\renewenvironment{Blue}{\color{blue}}{\color{black}}
%\renewenvironment{Emerald}{\special{color push Emerald}}{\special{color pop}}
%%\renewenvironment{Red}{\special{color push  Red}}{\special{color pop}}
%\renewenvironment{Red}{\color{red}}{\color{black}}
%\renewenvironment{Cyan}{\special{color push Cyan}}{\special{color pop}}
%\renewenvironment{textColor}[1]{\special{color push #1}}{\special{color pop}}
%\renewenvironment{Yellow}{\special{color push  Yellow}}{\special{color pop}}
%\renewenvironment{Black}{\special{color push  Black}}{\special{color pop}}
%\renewenvironment{Gray}{\special{color push  Gray}}{\special{color pop}}

